Turbo Training with Token Dropout

The objective of this paper is an efficient training method for video tasks. We make three contributions: (1) We propose Turbo training, a simple and versatile training paradigm for Transformers on multiple video tasks. (2) We illustrate the advantages of Turbo training on action classification, video-language representation learning, and long-video activity classification, showing that Turbo training can largely maintain competitive performance while achieving almost 4X speed-up and significantly less memory consumption. (3) Turbo training enables long-schedule video-language training and end-to-end long-video training, delivering competitive or superior performance than previous works, which were infeasible to train under limited resources.

==> table/action_classification.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lll|l}
\hline
Mask\%  & Recon\% & GFLOPs & UCF101 (top1)   \\ \hline
0 (normal finetune)   & -    & 180.6   & ?    \\\hline
50  & 50   & 99.3     & ?    \\
75  & 75   & 57.6     & ?    \\ 
75  & 25   & 45.9     & ?    \\ 
90  & 90   & 35.2     & ?    \\ 
90  & 10   & 18.3     & ?    \\ \hline
\end{tabular}
\caption{Speed and Performance trade-off of the UCF101 action classification task.}
\label{table:speed_acc}
\end{table}



\begin{figure}[!htb]
    \centering
    \begin{minipage}{0.6\textwidth}
        \centering
        \small
        \begin{tabular}{lll|ll}
        \hline
        Mask\%  & Recon\% & GFLOPs & UCF101 (top1) & HMDB51 (top1) \\ \hline
        0 (normal finetune)   & -    & 180.6   & ?    \\\hline
        50  & 50   & 99.3     & ?    \\
        75  & 75   & 57.6     & ?    \\ 
        75  & 25   & 45.9     & ?    \\ 
        90  & 90   & 35.2     & ?    \\ 
        90  & 10   & 18.3     & ?    \\ \hline
        \end{tabular}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
        \centering
        \small
        \begin{tabular}{c|c|c}
        \hline
           Method & Pretrain Data & R@1 \\ \hline
           CLIP (ViT-B-32)~\cite{Radford21} & YFCC & 16.8 \\
           MIL-NCE~\cite{Miech20} & HTM & 31.3 \\
           TAN~\cite{Han22TAN} & HTM & 49.4 \\ 
           \hline
           Ours (m=0.75,r=0.25) & HTM-AA & 36.7 \\
        \hline
        \end{tabular}
        % \caption{}
        % \label{table:pretrain}
    \end{minipage}
    \label{table:speed_acc}
    \caption{
    \textbf{Left}: Speed and Performance trade-off of the UCF101 action classification task.
    \textbf{Right}: Generalize to different mask ratios at the inference time.
    }
\end{figure}


==> table/coin.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{llll|l}
\hline
Temporal Method      & Clip Model       & Pretrain Supervision  & Pretrain Data & Acc (\%) \\ \hline
TSN (RGB+Flow)~\cite{Tang2019coin} & Inception        & [\cmark] action labels & K400 & 73.4    \\
% MIL-NCE     & S3D                 & [\xmark] MIL-NCE               & HTM  & 70.2    \\
Transformer~\cite{Feichtenhofer19} & SlowFast      & [\cmark] action labels & K400        & 71.6    \\ 
Transformer~\cite{Xu2021videoclip} & VideoCLIP     & [\xmark] NCE        & HTM            & 72.5    \\ 
% Transformer & TimeSformer   & [\cmark] action labels & K400        & 83.5    \\ 
Transformer~\cite{Lin22DistSup} & TimeSformer   & [\xmark] k-mean on ASR & HTM         & 85.3    \\
Transformer~\cite{Lin22DistSup} & TimeSformer   & [\xmark] Dist. Sup.    & HTM+WikiHow & 88.9    \\ \hline
\textbf{Turbo} $F_{16}$     & N/A (end-to-end)   & [\xmark] NCE & HTM-AA  & -  \\
\textbf{Turbo} $F_{32}$     & N/A (end-to-end)   & [\xmark] NCE & HTM-AA  & -    \\ 
\textbf{Turbo} $F_{64}$     & N/A (end-to-end)   & [\xmark] NCE & HTM-AA  & -       \\\hline
\end{tabular}
\caption{Procedural activitiy classification on the COIN dataset.}
\label{table:breakfast}
\end{table}

==> table/pretrain.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabu}{c|c|c}
        \hline
           Method & Pretrain Data & R@1 \\ \hline
           CLIP (ViT-B-32)~\cite{Radford21} & YFCC & 16.8 \\
           MIL-NCE~\cite{Miech20} & HTM & 31.3 \\
           \rowfont{\color{gray}}
           TAN~\cite{Han22TAN} & HTM & 49.4 \\ 
           \hline
           Ours (m=0.75, r=0.25) & HTM-AA & \textbf{36.7} \\
        \hline
    \end{tabu}
    \caption{
    Zero-shot text-visual alignment results on HTM-Align dataset. 
    We adopt the same setting as~\cite{Han22TAN} and report Recall@1 as the metric.}
    \label{tab:pretrain}
\end{table}







\begin{comment}
\begin{figure}[!htb]
    \centering
    \begin{minipage}{.35\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{images/vt.pdf}
        % \caption{}
        \label{fig:pretrain}
    \end{minipage}
    \begin{minipage}{0.55\textwidth}
        \centering
        \small
        \begin{tabular}{c|c|c}
        \hline
           Method & Pretrain Data & R@1 \\ \hline
           CLIP (ViT-B-32)~\cite{Radford21} & YFCC & 16.8 \\
           MIL-NCE~\cite{Miech20} & HTM & 31.3 \\
           TAN~\cite{Han22TAN} & HTM & 49.4 \\ 
           \hline
           Ours (m=0.75,r=0.25) & HTM-AA & 36.7 \\
        \hline
        \end{tabular}
        % \caption{}
        \label{table:pretrain}
    \end{minipage}
    \caption{\textbf{Left}: Progress of vision-language pretraining monitor by R@1 on HTM-Align dataset.
    \textbf{Right}: Zero-shot text-visual alignment results on HTM-Align dataset. We report R@1 as the metric.
    }
\end{figure}
\end{comment}

==> table/supp_alignment.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabu}{c|c|c|c|c}
        \hline
           Method & Arch. & Pretrain Data & Temporal R.F. & R@1 \\ \hline
           CLIP~\cite{Radford21} & ViT-B-32 & YFCC & 1s & 16.8 \\
           CLIP~\cite{Radford21} & ViT-B-16 & YFCC & 1s & 22.0 \\
           MIL-NCE~\cite{Miech20} & S3D-G & HTM & 1s & 31.3 \\
           \rowfont{\color{gray}}
           TAN$^{*}$~\cite{Han22TAN} & S3D-G \& TFM  & HTM & 64s & 49.4 \\ 
           NCE with TAN$^{\dag}$~\cite{Han22TAN} & S3D-G & HTM-AA  & 1s. & {33.6} \\
           \hline
           Ours (m=0.75, r=0.25) & ViT-B-16 & HTM-AA & 1s & \textbf{36.7} \\
        \hline
    \end{tabu}
    \caption{
    Zero-shot text-visual alignment results on HTM-Align dataset. 
    We adopt the same setting as~\cite{Han22TAN} and report Recall@1 as the metric.
    $*$: result from TAN is not directly comparable
    because their model contains transformers (TFM) on S3D-G features that takes a much longer temporal context for the temporal alignment task. This table provides additional comparisons and details over Table~3 (right) in the main paper.
    $\dag$: we train the NCE loss on HTM-AA for the same duration (approx. 60h) for a fair comparison. 
    }
    \label{tab:supp_pretrain}
    \vspace{-5mm}
\end{table}

